Exploiting Regional Information Transformer for Single Image Deraining

Transformer-based Single Image Deraining (SID) methods have achieved remarkable success, primarily attributed to their robust capability in capturing long-range interactions. However, we've noticed that current methods handle rain-affected and unaffected regions concurrently, overlooking the disparities between these areas, resulting in confusion between rain streaks and background parts, and inabilities to obtain effective interactions, ultimately resulting in suboptimal deraining outcomes. To address the above issue, we introduce the Region Transformer (Regformer), a novel SID method that underlines the importance of independently processing rain-affected and unaffected regions while considering their combined impact for high-quality image reconstruction. The crux of our method is the innovative Region Transformer Block (RTB), which integrates a Region Masked Attention (RMA) mechanism and a Mixed Gate Forward Block (MGFB). Our RTB is used for attention selection of rain-affected and unaffected regions and local modeling of mixed scales. The RMA generates attention maps tailored to these two regions and their interactions, enabling our model to capture comprehensive features essential for rain removal. To better recover high-frequency textures and capture more local details, we develop the MGFB as a compensation module to complete local mixed scale modeling. Extensive experiments demonstrate that our model reaches state-of-the-art performance, significantly improving the image deraining quality. Our code and trained models are publicly available.

==> section/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bio/BLi.jpeg}}]{Baiang Li}  received his B.E. degree from Hefei University of Technology, Hefei, China in 2024. His research interests include computational photography, image processing and generative model. He has published papers in ACM MM, ACM Siggraph and CVPR Workshop, and he has been acting as a reviewer of CVPR, ECCV and ACM MM.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bio/zzhang.png}}]{Zhao Zhang} (SM’17-) is a Full Professor at the School of Computer Science and Information Engineering, Hefei University of Technology, Hefei, China. He received a Ph.D. degree from City University of Hong Kong in 2013. His research interests include Machine Learning \& Data Mining, Pattern Recognition \& Image Processing. He has authored/co-authored more than 130 technical papers published at prestigious journals and conferences, including 33 IEEE/ACM Transactions papers. Dr. Zhang is serving as an Associate Editor of IEEE Transactions on Image Processing and Elsevier Pattern Recognition. He has been acting as a Senior PC member/Area Chair of IJCAI,SDM,ECAI,BMVC, and PAKDD. He is a Senior Member of IEEE. 
\end{IEEEbiography} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bio/huan.jpg}}]{Huan Zheng}
received her B.E. degree from Northwest Agriculture and Forestry University (NWAFU). Currently, he is working toward the master’s degree with the School of Computer Science and Information Engineering, Hefei University of Technology (HFUT). His research interests include Deep Learning and Computer Vision, Image/Video Restoration and Enhancement.
\end{IEEEbiography} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bio/xxu.jpeg}}]{Xiaogang Xu} is a research fellow in the Chinese University of Hong Kong. He obtained his Ph.D. degree from the Chinese University of Hong Kong in 2022. He received his bachelor degree from Zhejiang University. He obtained the Hong Kong PhD Fellowship in 2018. He serves as a reviewer for CVPR, ICCV, ECCV, AAAI, ICLR, Neurips, TPAMI, IJCV. His research interest includes deep generative networks, low-level vision, etc.
\end{IEEEbiography} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bio/ywei.png}}]{Yanyan Wei} is a Lecturer at the School of Computer Science and Information Engineering, Hefei University of Technology. He received a Ph.D. degree from Hefei University of Technology in 2022. His research interests include Deep Learning and Computer Vision, Image/Video Restoration and Enhancement.
\end{IEEEbiography} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bio/zjy.jpg}}]{Jingyi Zhang} received her B.E. degree from Hefei University of Technology, Hefei, China, in 2024. 
% Currently, she serves as a research assistant at the Tianjin Key Laboratory of Visual Computing and Intelligent Perception. 
Her research interests include image generation and image processing, such as image super-resolution and image restoration. She is currently involved in the submission of two research papers.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bio/jfan.png}}]{Jicong Fan} is an Assistant Professor at the School of Data Science, The Chinese University of Hong Kong, Shenzhen. His research results have been published in IEEE TSP/TNNLS/TII, KDD, NeurIPS, CVPR, ICLR, ICML, AAAI. He is a senior member of IEEE and currently serves as an associate editor of the journals Pattern Recognition and Neural Processing Letters. He won the first prize of the 2023 Natural Science Award of the Chinese Automation Society and was selected into Stanford University's 2023 "Top 2\% Global Scientists" list.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip]{bio/mwang.jpeg}}]{Meng Wang} is a professor at Hefei University of Technology, China. He received the B.E. degree and Ph.D. degree in the Special Class for the Gifted Young and the Department of Electronic Engineering and Information Science from the University of Science and Technology of China (USTC), Hefei, China, in 2003 and 2008, respectively. He received paper prizes or awards from ACM MM 2009 (Best Paper Award), ACM MM 2010 (Best Paper Award), ACM MM 2012 (Best Demo Award), ICDM 2014 (Best Student Paper Award), SIGIR 2015 (Best Paper Honorable Mention), IEEE TMM 2015 and 2016 (Prize Paper Award Honorable Mention), IEEE SMC 2017 (Best Transactions Paper Award), and ACM TOMM 2018 (Nicolas D. Georganas Best Paper Award). He is or has been an editorial board member of IEEE Trans. on Circuits and Systems for Video Technology, IEEE Trans. on Multimedia, IEEE Trans. on Knowledge and Data Engineering, IEEE Trans. on Neural Networks and Learning Systems, etc. He is now a Fellow of the IEEE. 
\end{IEEEbiography}
